Understanding the Ability of LLMs to Handle Character-Level Perturbation

This work investigates the resilience of contemporary large language models (LLMs) against frequent character-level perturbations. We examine three types of character-level perturbations including introducing numerous typos within words, shuffling the characters in each word, and inserting a large number of invisible characters into the text. Surprisingly, even under severe perturbation, such as shuffling nearly all words character-wise to produce text that is almost unreadable to humans, or inserting invisible characters which are several times more than the visible ones as noise, many LLMs still maintain notable performance. We explore the underlying causes of this robustness and find that LLMs exhibit remarkable resilience to chaotic segmentation and fragmented tokenization. Furthermore, we examine the mechanisms by which LLMs remove perturbations to correctly comprehend text, including both implicit and explicit mechanisms for character-level perturbation. We hope that our findings on the low-level robustness of LLMs will unveil their inherent architectural strengths, reveal the potential risks of their misuse, and inform the reliable deployment of LLMs across diverse application scenarios.

==> content/Factors_Influencing_the_Performance_of_LLMs/different_obfuscated_format.tex <==
\subsection{Different Obfuscated Format}

\subsubsection{Use Star(*) to Replace VS Characters}
\begin{tikzpicture}
\begin{axis}[
    title={replacing VSs with stars},
    xlabel={inserted\_noise\_cnt},
    ylabel={accuracy\_rate},
    xmin=0, xmax=3,
    ymin=0, ymax=1,
    xtick={0,1,2,3},
    grid=both,
    grid style={line width=.1pt, draw=gray!30},
    major grid style={line width=.2pt,draw=gray!50},
    legend style={cells={anchor=west}, legend pos=north east},
    width=0.9\textwidth,
    height=8cm,
    cycle list name=exotic,  % 启用自动颜色分配
]

% 第一条折线
\addplot+[
    line width=1.5pt
] table[x=code_cnt, y=score] {exp9_qwen3-30B-normal.dat};
\addlegendentry{Qwen3(30B)(star)-nothinking}

\addplot+[
    line width=1.5pt
] table[x=code_cnt, y=score] {exp3_qwen3-30B-normal.dat};
\addlegendentry{Qwen3(30B)(VS)-nothinking}

\addplot+[
    line width=1.5pt
] table[x=code_cnt, y=score] {exp9_qwen3-30B-thinking.dat};
\addlegendentry{Qwen3(30B)(star)-thinking}

% 第二条折线
\addplot+[
    line width=1.5pt
] table[x=code_cnt, y=score] {exp3_qwen3-30B-thinking.dat};
\addlegendentry{Qwen3(30B)(VS)-thinking}


\end{axis}
\end{tikzpicture}

The distribution of similar polylines are different.


\subsubsection{Use Character 'A' to Replace VS Characters}

\begin{tikzpicture}
\begin{axis}[
    title={replacing VSs with 'A'},
    xlabel={inserted\_noise\_cnt},
    ylabel={accuracy\_rate},
    xmin=0, xmax=3,
    ymin=0, ymax=1,
    xtick={0,1,2,3},
    grid=both,
    grid style={line width=.1pt, draw=gray!30},
    major grid style={line width=.2pt,draw=gray!50},
    legend style={cells={anchor=west}, legend pos=north east},
    width=0.9\textwidth,
    height=8cm,
    cycle list name=exotic,  % 启用自动颜色分配
]

% 第一条折线
\addplot+[
    line width=1.5pt
] table[x=code_cnt, y=score] {exp9_qwen3-30B-A-normal.dat};
\addlegendentry{Qwen3(30B)(A)-nothinking}

\addplot+[
    line width=1.5pt
] table[x=code_cnt, y=score] {exp3_qwen3-30B-normal.dat};
\addlegendentry{Qwen3(30B)(VS)-nothinking}

\addplot+[
    line width=1.5pt
] table[x=code_cnt, y=score] {exp9_qwen3-30B-A-thinking.dat};
\addlegendentry{Qwen3(30B)(A)-thinking}

% 第二条折线
\addplot+[
    line width=1.5pt
] table[x=code_cnt, y=score] {exp3_qwen3-30B-thinking.dat};
\addlegendentry{Qwen3(30B)(VS)-thinking}

\end{axis}
\end{tikzpicture}

\subsubsection{Use Visible ASCII Characters to Replace VS Characters}

\begin{tikzpicture}
\begin{axis}[
    title={replacing VSs with Visible ASCII Characters},
    xlabel={inserted\_noise\_cnt},
    ylabel={accuracy\_rate},
    xmin=0, xmax=3,
    ymin=0, ymax=1,
    xtick={0,1,2,3},
    grid=both,
    grid style={line width=.1pt, draw=gray!30},
    major grid style={line width=.2pt,draw=gray!50},
    legend style={cells={anchor=west}, legend pos=north east},
    width=0.9\textwidth,
    height=8cm,
    cycle list name=exotic,  % 启用自动颜色分配
]

% 第一条折线
\addplot+[
    line width=1.5pt
] table[x=code_cnt, y=score] {exp10_qwen3-30B-N-normal.dat};
\addlegendentry{Qwen3(30B)(small set)-nothinking}

\addplot+[
    line width=1.5pt
] table[x=code_cnt, y=score] {exp10_qwen3-30B-N-thinking.dat};
\addlegendentry{Qwen3(30B)(small set)-thinking}

\addplot+[
    line width=1.5pt
] table[x=code_cnt, y=score] {exp10_qwen3-30B-W-normal.dat};
\addlegendentry{Qwen3(30B)(big set)-nothinking}

\addplot+[
    line width=1.5pt
] table[x=code_cnt, y=score] {exp10_qwen3-30B-W-thinking.dat};
\addlegendentry{Qwen3(30B)(big set)-thinking}


\addplot+[
    line width=1.5pt
] table[x=code_cnt, y=score] {exp3_qwen3-30B-normal.dat};
\addlegendentry{Qwen3(30B)(VS)-nothinking}
\addplot+[
    line width=1.5pt
] table[x=code_cnt, y=score] {exp3_qwen3-30B-thinking.dat};
\addlegendentry{Qwen3(30B)(VS)-thinking}
\end{axis}
\end{tikzpicture}


==> content/Factors_Influencing_the_Performance_of_LLMs/method.tex <==






==> content/discuss/Explicit_Denoising.tex <==
\subsection{Explicit Denoising}


To further investigate the model's capacity for explicit denoising, we introduced instructions in the prompt that explicitly required the model to remove noise from the input text before generating an answer. This setup was designed to manually activate and evaluate the model’s explicit denoising behavior. We conducted experiments using the Qwen3-30B (A3B) model on the GSM8K dataset under this prompted denoising condition. The corresponding results are presented in Table \ref{tab:prompted_to_denoise}.

\begin{table}[ht]
    
\caption{Prompted to denoise the statement} % 可选标题

\label{tab:prompted_to_denoise} % 可选标签

\begin{center}
\begin{tabular}{c|c|cccc}
\toprule
\bf{Model Name} & \textbf{Whether to Prompt} & \textbf{Baseline} &  \textbf{1}&  \textbf{2}&  \textbf{3}\\
\midrule
\multirow{2}{*} {Qwen3-30B(A3B)(Thinking) }& Yes & 0.956 & 0.728 & 0.100 & 0.030 \\
& No & 0.956 & 0.575 & 0.070 & 0.022 \\
\midrule
\multirow{2}{*} {Qwen3-30B(A3B)(Normal) }& Yes & 0.941 & 0.660 & 0.095 & 0.031 \\
& No & 0.941 & 0.434 & 0.047 & 0.026 \\
\bottomrule
\end{tabular}\\
\footnotesize
1,2 and 3 means the number of inserted VS characters attached to each visible character.\\
'Normal' means add 'nothink' token to prevent models from long reasoning, but there is still a brief chain of thought

\end{center}
\end{table}

Table \ref{tab:prompted_to_denoise} indicates that models has certain difficulty to explicitly denoise the given text, especially in the case of inserting more than one VSs attaching to normal characters.

Furthermore, we provided few-shot examples to help models follow the instructions, as shown in Figure \ref{fig:prompted_to_denoise_shots}, indicating that models still give a poor performance in explicit denoising. 
\begin{figure}[ht]
    \centering
    \begin{tikzpicture}
    \begin{axis}[
        ylabel={accuracy\_rate},
        xlabel={inserted\_noise\_cnt},
        xmin=1, xmax=3,
        ymin=0, ymax=1,
        xtick={0,1,2,3},
        grid=both,
        grid style={line width=.1pt, draw=gray!30},
        major grid style={line width=.2pt,draw=gray!50},
        legend style={cells={anchor=west}, legend pos=north east},
        width=0.9\textwidth,
        height=8cm,
        cycle list name=exotic,
    ]
    \addplot+[
        line width=1.5pt
    ] table[x=code_cnt, y=score] {exp3_qwen3-30B-normal.dat};
    \addlegendentry{no prompt}
    \addplot+[
        line width=1.5pt
    ] table[x=code_cnt, y=score] {exp15_shot0.dat};
    \addlegendentry{0-shot}
    
    \addplot+[
        line width=1.5pt
    ] table[x=code_cnt, y=score] {exp15_shot1.dat};
    \addlegendentry{1-shots}
    \addplot+[
        line width=1.5pt
    ] table[x=code_cnt, y=score] {exp15_shot2.dat};
    \addlegendentry{2-shots}
    
    \addplot+[
        line width=1.5pt
    ] table[x=code_cnt, y=score] {exp15_shot3.dat};
    \addlegendentry{3-shots}
    \addplot+[
        line width=1.5pt
    ] table[x=code_cnt, y=score] {exp15_shot4.dat};
    \addlegendentry{4-shots}
    \end{axis}
    \end{tikzpicture}
    %\vspace{\baselineskip} 
    \caption{Prompted to denoise the statement with few shots(Qwen3-30B(A3B)-Normal)}
    \label{fig:prompted_to_denoise_shots}
\end{figure}

We analyzed the model's performance in conducting explicit denoising within its chain of thought (CoT)\citep{wei2023chainofthoughtpromptingelicitsreasoning} under varying levels of inserted noise and numbers of few-shot examples. The model’s CoT outputs were categorized into three types:

\begin{enumerate}[label=\textbf{\Alph*.}]
\item The model correctly outputs clean (noise-free) text during its response (meaning preserved), followed by the reasoning process and an answer (regardless of the answer's correctness).
\item The model attempts to output clean text during its response, but the resulting denoised text contains errors or misses critical information compared to the original, followed by the reasoning process and an answer (regardless of the answer's correctness).
\item The model does not explicitly output clean text at all, and instead directly provides the reasoning process and an answer (or only an answer without explicit reasoning).
\end{enumerate}

We examined the responses with a total output length of no more than 10,000 characters and calculated the proportions of these three categories, as shown in Figure \ref{fig:statistics} and \ref{fig:statistics2}.


\begin{figure}[htp]
    
    \begin{minipage}{0.32\textwidth}
    \begin{tikzpicture}
    %291 583 425
    \pie[radius=1.5, text=legend]{22.4/A, 44.9/B, 32.7/C}
    \node[above, font=\small, yshift=2cm]{No prompted, no thinking};
    \end{tikzpicture}
    \end{minipage}
    \hfill
    \begin{minipage}{0.32\textwidth}
    \begin{tikzpicture}
    %19 783 465
    \pie[radius=1.5, text=legend]{1.5/A, 63.8/B, 34.6/C}
    \node[above, font=\small, yshift=2cm]{No prompted, no thinking};
    \end{tikzpicture}
    \end{minipage}
    \hfill
    \begin{minipage}{0.32\textwidth}
    \begin{tikzpicture}
    %2 523 732
    \pie[radius=1.5, text=legend]{0.2/A, 41.6/B, 58.2/C}
    \node[above, font=\small, yshift=2cm]{No prompted, no thinking};
    \end{tikzpicture}
    \end{minipage}
    
    \begin{minipage}{0.32\textwidth}
    \begin{tikzpicture}
    %247 495 395
    \pie[radius=1.5, text=legend]{21.7/A, 43.5/B, 34.7/C}
    \node[above, font=\small, yshift=2cm]{No prompted, thinking};
    \end{tikzpicture}
    \end{minipage}
    \hfill
    \begin{minipage}{0.32\textwidth}
    \begin{tikzpicture}
    %1 159 847
    \pie[radius=1.5, text=legend]{0.1/A, 15.8/B, 84.1/C}
    \node[above, font=\small, yshift=2cm]{No prompted, thinking};
    \end{tikzpicture}
    \end{minipage}
    \hfill
    \begin{minipage}{0.32\textwidth}
    \begin{tikzpicture}
    %7 162 868
    \pie[radius=1.5, text=legend]{0.7/A, 15.6/B, 83.7/C}
    \node[above, font=\small, yshift=2cm]{No prompted, thinking};
    \end{tikzpicture}
    \end{minipage}

    \begin{minipage}{0.32\textwidth}
    \begin{tikzpicture}
    %1059 222 7
    \pie[radius=1.5, text=legend]{82.2/A, 17.2/B, 0.5/C}
    \node[above, font=\small, yshift=2cm]{Prompted, no thinking};
    \end{tikzpicture}
    \end{minipage}
    \hfill
    \begin{minipage}{0.32\textwidth}
    \begin{tikzpicture}
    %128 980 38
    \pie[radius=1.5, text=legend]{11.2/A, 85.5/B, 3.3/C}
    \node[above, font=\small, yshift=2cm]{Prompted, no thinking};
    \end{tikzpicture}
    \end{minipage}
    \hfill
    \begin{minipage}{0.32\textwidth}
    \begin{tikzpicture}
    %56 941 70
    \pie[radius=1.5, text=legend]{5.2/A, 88.2/B, 6.6/C}
    \node[above, font=\small, yshift=2cm]{Prompted, no thinking};
    \end{tikzpicture}
    \end{minipage}
    
    \begin{minipage}{0.32\textwidth}
    \begin{tikzpicture}
    %993 142 38
    \pie[radius=1.5, text=legend]{84.7/A, 12.1/B, 3.2/C}
    \node[above, font=\small, yshift=2cm]{Prompted, thinking};
    \end{tikzpicture}
    \end{minipage}
    \hfill
    \begin{minipage}{0.32\textwidth}
    \begin{tikzpicture}
    %198 191 246
    \pie[radius=1.5, text=legend]{31.2/A, 30.1/B, 38.7/C}
    \node[above, font=\small, yshift=2cm]{Prompted, thinking};
    \end{tikzpicture}
    \end{minipage}
    \hfill
    \begin{minipage}{0.32\textwidth}
    \begin{tikzpicture}
    %83 174 318
    \pie[radius=1.5, text=legend]{14.4/A, 30.3/B, 55.3/C}
    \node[above, font=\small, yshift=2cm]{Prompted, thinking};
    \end{tikzpicture}
    \end{minipage}

    \begin{minipage}{0.32\textwidth}
    \begin{tikzpicture}
    %1148 163 1
    \pie[radius=1.5, text=legend]{87.5/A, 12.4/B, 0.1/C}
    \node[above, font=\small, yshift=2cm]{1-shot, no thinking};
    \end{tikzpicture}
    \end{minipage}
    \hfill
    \begin{minipage}{0.32\textwidth}
    \begin{tikzpicture}
    %257 1030 0
    \pie[radius=1.5, text=legend]{20.0/A, 80.0/B, 0.0/C}
    \node[above, font=\small, yshift=2cm]{1-shot, no thinking};
    \end{tikzpicture}
    \end{minipage}
    \hfill
    \begin{minipage}{0.32\textwidth}
    \begin{tikzpicture}
    %72 1222 1
    \pie[radius=1.5, text=legend]{5.6/A, 94.4/B, 0.1/C}
    \node[above, font=\small, yshift=2cm]{1-shot, no thinking};
    \end{tikzpicture}
    \end{minipage}
    \caption{The proportions of three categories on Qwen3-30B(A3B). One line from left to right refers to noise count 1,2,3. }
    \label{fig:statistics}
\end{figure}

\begin{figure}[htp]
    
    \begin{minipage}{0.32\textwidth}
    \begin{tikzpicture}
    %2 62 1249
    \pie[radius=1.5, text=legend]{0.2/A, 4.7/B, 95.1/C}
    \node[above, font=\small, yshift=2cm]{No prompted};
    \end{tikzpicture}
    \end{minipage}
    \hfill
    \begin{minipage}{0.32\textwidth}
    \begin{tikzpicture}
    %34 315 955
    \pie[radius=1.5, text=legend]{2.6/A, 24.2/B, 73.2/C}
    \node[above, font=\small, yshift=2cm]{prompted};
    \end{tikzpicture}
    \end{minipage}
    \hfill
    \begin{minipage}{0.32\textwidth}
    \begin{tikzpicture}
    %663 641 0
    \pie[radius=1.5, text=legend]{50.8/A, 49.2/B, 0.0/C}
    \node[above, font=\small, yshift=2cm]{1-shot};
    \end{tikzpicture}
    \end{minipage}
    
    \caption{The proportions of three categories of LLama3.1-70B when inserting one noise attached to each visible character}
    \label{fig:statistics2}
\end{figure}

For case inserting one noise character after each visible character, we further calculated the percentage of correct and incorrect samples in the three types relative to the total number of samples, as shown in the Table \ref{tab:correct and wrong percentage}. Furthermore, there are 196 problems(about 15\%) give wrong answer with answer type C in the case no prompted, while give correct answer with type A in the case of 1 shot; the accuracy of LLama3.1-70B increased from 10\%(no prompted) to 51\%(1-shot). This indicates that explicit denoising is an effective method for models to reorganize information and provide correct answers. 


\begin{table}
\begin{center}
\caption{Percentage of correct and incorrect samples in the three types} % 可选标题
\label{tab:correct and wrong percentage} % 可选标签
\begin{tabular}{c|ccc|ccc|ccc|}

\toprule
\multirow{2}{*} {Strategy}& \multicolumn{3}{c|}{A} &  \multicolumn{3}{c|}{B} & \multicolumn{3}{c|}{C}  \\
&  correct & wrong & total & total & wrong &total&correct & wrong&total \\

\midrule
no prompted & 20.9\% & 1.5\% & 22.4\% & 12.5\% & 32.4\% & 44.9\% & 10.9\% & 21.8\% & 32.7\%\\

\midrule
prompted & 62.7\% & 19.5\% & 82.2\% & 4.8\% & 12.4\% & 17.2\% & 0.0\% & 0.5\% & 0.5\%\\
\midrule
1-shot & 74.3\% & 13.2\% & 87.5\% & 4.9\% & 7.5\% & 12.4\% & 0.0\% & 0.1\% & 0.1\%\\
\bottomrule
\end{tabular}\\


\end{center}
\end{table}

==> content/discuss/High-level_Denoising.tex <==
\subsection{High-level Denoising}
\label{sec:method}

To understand models' high-level denoising behavior, that is, the explicit denoising of input text through the process of CoT reasoning, we address three natural questions:

\begin{enumerate}
\item Does the model rearrange and reconstruct the clean text through the CoT process?
\item Does the CoT process help models comprehend the problem more effectively?
\item Is the reconstruction of clean text an explicit rule-based procedure (meaning the model recognizes the noise pattern and follows a deterministic rule, such as copying characters at fixed intervals) or an implicit one?
\end{enumerate}

To investigate the first question, we calculated the proportion of responses containing explicit denoising across all questions. The model’s CoT outputs were categorized into three types:

\begin{enumerate}[label=\textbf{\Alph*.}]
\item The model correctly produces clean (noise-free) text during its response (preserving the original meaning), followed by a reasoning process and an answer (regardless of correctness).
\item The model attempts to produce clean text, but the denoised output contains errors or omits critical information compared to the original, followed by a reasoning process and an answer (regardless of correctness).
\item The model does not explicitly output clean text and directly provides a reasoning process and an answer (or only an answer without explicit reasoning).
\end{enumerate}

We analyzed the responses on GSM8K from the Qwen3-30B(A3B) model in no-thinking mode, using an LLM to assist in categorizing the CoT outputs according to the above criteria. For \inj{1}, 55.1\% of Qwen3's responses fell into category A or B. This indicates that \textbf{models do use CoT to rearrange and reconstruct clean text}.

To examine whether the CoT process aids models in better comprehending the problem, we incorporated instructions in the prompt explicitly directing the model to remove noise from the input before generating an answer. The models' accuracy on GSM8K is shown in Table \ref{tab:prompted_to_denoise}. We also provided a one-shot example and calculated the percentage of correct and incorrect responses across the three categories under \inj{1}, as shown in Table \ref{tab:correct and wrong percentage}. The results show that the proportion of type A and B responses increased with prompted denoising and one-shot guidance, alongside an improvement in accuracy. For instance, the accuracy of the thinking model under \inj{1} increased from 57.5\% to 72.8\%. Furthermore, there are 196 problems(about 15\%) gave wrong answer with type C in the case no prompted, while gave correct answer with type A in the case of 1 shot. This suggests that \textbf{the CoT process does help models comprehend the problem more effectively}.

\begin{table}[ht]
\begin{center}
\caption{Prompted to denoise the statement}
\label{tab:prompted_to_denoise} 
\begin{tabular}{c|c|cccc}
\toprule
\bf{Model Name} & \textbf{Whether to Prompt} & \textbf{Baseline} &  \textbf{\inj{1}}&  \textbf{\inj{2}}&  \textbf{\inj{3}}\\
\midrule
\multirow{2}{*} {Qwen3-30B(A3B)(Thinking) }& Yes & 0.956 & \textbf{0.728} & \textbf{0.100} & \textbf{0.030} \\
& No & 0.956 & 0.575 & 0.070 & 0.022 \\
\midrule
\multirow{2}{*} {Qwen3-30B(A3B)(Normal) }& Yes & 0.941 & \textbf{0.660} & \textbf{0.095} & \textbf{0.031} \\
& No & 0.941 & 0.434 & 0.047 & 0.026 \\
\bottomrule
\end{tabular}\\
\end{center}
\end{table}

\begin{center}
\begin{table}[ht]
\caption{Percentage of correct and incorrect samples in the three types} % 可选标题
\label{tab:correct and wrong percentage} % 可选标签
\begin{tabular}{c|ccc|ccc|ccc}

\toprule
\multirow{2}{*} {Strategy}& \multicolumn{3}{c|}{A} &  \multicolumn{3}{c|}{B} & \multicolumn{3}{c}{C}  \\
&  correct & wrong & total & total & wrong &total&correct & wrong&total \\

\midrule
no prompted & 20.9\% & 1.5\% & 22.4\% & 12.5\% & 32.4\% & 44.9\% & 10.9\% & 21.8\% & 32.7\%\\

\midrule
prompted & 62.7\% & 19.5\% & 82.2\% & 4.8\% & 12.4\% & 17.2\% & 0.0\% & 0.5\% & 0.5\%\\
\midrule
1-shot & 74.3\% & 13.2\% & 87.5\% & 4.9\% & 7.5\% & 12.4\% & 0.0\% & 0.1\% & 0.1\%\\
\bottomrule
\end{tabular}\\

\end{table}
\end{center}

We examined the tokens in the model's CoT responses and observed that the output tokens are word-wise. For example, given a perturbed token sequence such as [t, ?, h, ?, e, ?], the model directly outputs the word the as a single token, rather than generating three separate character-level tokens [t, h, e]. This behavior persisted even when we manually applied character-level tokenization to the response in the one-shot example. These findings indicate that \textbf{the reconstruction of clean text is not a rule-based procedure}. Instead, the model leverages underlying low-level capabilities to directly infer word-level meaning from the noisy text beforehand. The CoT process then serves primarily to reorganize this information, without performing additional comprehension at the level of word semantics.
% \input{content/discuss/Explicit Denoising}

==> content/discuss/Implicit_Denoising.tex <==
%\subsubsection{Implicit Denoising}

As mentioned above, even when explicitly prompted to output clean text first, the model consistently produces clean text using word-level tokens rather than character-level tokens. This suggests that the model comprehends the meaning of words within the noise-perturbed text even before generating the clean output. We therefore hypothesize that the model employs a non-procedural, implicit denoising mechanism: as the input is processed layer by layer, the model gradually learns to focus primarily on the non-noise characters in the text, thereby recovering their semantic information.

To further validate this, we selected several longer problem instances and, for each prefix ending with a complete word, computed the average cosine similarity of the hidden states (across all layers except the last) between the model's processing of the text with and without inserted noise. The similarity trends for a sample problem are illustrated in Figure \ref{fig:similarity}.

Figure \ref{fig:similarity} shows that the hidden states exhibit high similarity between clean and noisy inputs, indicating that \textbf{the model possesses internal mechanisms to implicitly denoise the text and recover underlying meanings}. Furthermore, the similarity tends to decrease as the prefix length increases, suggesting that \textbf{this mechanism is implicit and unstable, rather than a deterministic or programmatic procedure}.

\begin{figure}[ht]
    \centering
    \begin{tikzpicture}
    \begin{axis}[
        ylabel={Similarity},
        xlabel={Prefix word count},
        xmin=1, xmax=90,
        ymin=0.7, ymax=0.9,
        grid=both,
        grid style={line width=.1pt, draw=gray!30},
        major grid style={line width=.2pt,draw=gray!50},
        legend style={cells={anchor=west}, legend pos=north east},
        width=0.9\textwidth,
        height=8cm,
        cycle list name=exotic,
    ]
    \addplot[
        only marks,
        mark=*,
        mark size=1.5pt,
        red
    ] table {exp6_problem1.dat};
    \addplot[
        domain=0:90,
        thick,
        blue
    ] {-0.0006713588442688128*x+0.8275520033475642};
    \end{axis}
    \end{tikzpicture}
    %\vspace{\baselineskip} 
    \caption{Prompted to denoise the statement with few shots(Qwen3-30B(A3B)-Normal)}
    \label{fig:similarity}
\end{figure}


==> content/discuss/Low-level_Denoising.tex <==
\subsection{Low-level Denoising}

We then investigated the models' low-level denoising ability to comprehend word meanings from noisy and fragmented token sequences.

We observed that, regardless of how models remove noise from the input text, a critical step involves recognizing the original meaning of a word from its separated character-level tokens. Thus, we break down the models' low-level denoising ability into two aspects: (1) the ability to understand the meaning of words under fragmented tokenization caused by inserted noise, and (2) the ability to remove noise from token sequences.

%\input{content/discuss/Comprehend Under Character-Level Tokenization}

\input{content/discuss/Implicit Denoising}

==> content/discuss/discuss.tex <==
\section{Mechanism behind Robustness of Denoising}
\label{sec:breakdown}

In this section, we investigate the underlying mechanisms through which language models comprehend inputs perturbed by noise characters. We break down models' behavior of denoising into two aspects: (i) high-level denoising: to rearrange and reconstruct clean text from noisy input text through an explicit Chain-of-Thought (CoT)~\citep{wei2023chainofthoughtpromptingelicitsreasoning} process; (ii) low-level denoising: to comprehend words' meanings from noisy and fragmented token sequences in word level.\says{zay}{need to maintain?}{blue}

\input{content/discuss/High-level_Denoising}
\input{content/discuss/Low-level_Denoising}


==> content/rec.tex <==
% 第二个子图 - 移除图例
    % \begin{subfigure}{0.33\textwidth}
    %     \centering
    %     \begin{tikzpicture}
    %     \begin{axis}[
    %         title={Reading Comprehension},
    %         % ylabel={score},
    %         xlabel={inserted\_code\_cnt},
    %         xmin=0, xmax=3,
    %         ymin=0, ymax=5,
    %         xtick={0,1,2,3},
    %         grid=both,
    %         grid style={line width=.1pt, draw=gray!30},
    %         major grid style={line width=.2pt,draw=gray!50},
    %         width=\textwidth,
    %         height=4cm,
    %         cycle list name=exotic,
    %         legend style={draw=none, fill=none, cells={anchor=west}, font=\small},
    %         %legend pos=outer north east,
    %     ]
    %     \addplot+[line width=1.5pt] table[x=code_cnt, y=score] {exp2_dsv3.dat};
        
    %     \addplot+[line width=1.5pt] table[x=code_cnt, y=score] {exp2_dsr1.dat};
        
    %     \addplot+[line width=1.5pt] table[x=code_cnt, y=score] {exp2_Qwen3-235B-normal.dat};
        
    %     \addplot+[line width=1.5pt] table[x=code_cnt, y=score] {exp2_Qwen3-235B-Thinking.dat};
        
    %     \addplot+[line width=1.5pt] table[x=code_cnt, y=score] {exp2_Qwen3-30B-normal.dat};
    %     \label{plot:qwen30b}
        
    %     \addplot+[line width=1.5pt] table[x=code_cnt, y=score] {exp2_Qwen3-30B-thinking.dat};
    %     \label{plot:qwen30b_thinking}
    %     \end{axis}
    %     \end{tikzpicture}
    % \end{subfigure}
    % \hfill

==> datas/exp5.tex <==





==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

